End-to-end verifiable voting for developing countries -- what's hard in Lausanne is harder still in Lahore

In recent years end-to-end verifiable voting (E2EVV) has emerged as a promising new paradigm to conduct evidence-based elections. However, E2EVV systems thus far have primarily been designed for the developed world and the fundamental assumptions underlying the design of these systems do not readily translate to the developing world, and may even act as potential barriers to adoption of these systems. This is unfortunate because developing countries account for 80\% of the global population, and given their economic and socio-political dilemmas and their track record of contentious elections, these countries arguably stand to benefit most from this exciting new paradigm. In this paper, we highlight various limitations and challenges in adapting E2EVV systems to these environments, broadly classed across social, political, technical, operational, and human dimensions. We articulate corresponding research questions and identify significant literature gaps in these categories. We also suggest relevant strategies to aid researchers, practitioners, and policymakers in visualizing and exploring solutions that align with the context and unique ground realities in these environments. Our goal is to outline a broader research agenda for the community to successfully adapt E2EVV voting systems to developing countries.

==> important_thoughts.tex <==
- vVote, had to change candidate name ordering, Scantegrity had to devise dispute resolution process, other papers have also noted practical concerns - e.g. key management in Helios trials
%Sastry has noted that discarded receipts can be an attack vector

Also focus on non-process factors
